A Log-Sensitive Encoding of Turing Machines in the $\lambda$-Calculus

This note modifies the reference encoding of Turing machines in the $\lambda$-calculus by Dal Lago and Accattoli, which is tuned for time efficiency, as to accommodate logarithmic space. There are two main changes: Turing machines now have *two* tapes, an input tape and a work tape, and the input tape is encoded differently, because the reference encoding comes with a linear space overhead for managing tapes, which is excessive for studying logarithmic space.

==> latex-macros/ben-macros-diagrams.tex <==
\usepackage{tikz}
\makeatletter
\protected\def\tikz@nonactivecolon{\ifmmode\mathrel{\mathop\ordinarycolon}\else:\fi} 
\makeatother

\usetikzlibrary{matrix,arrows}
\usetikzlibrary{decorations.shapes}
\usetikzlibrary{decorations.text}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{arrows.meta}

%\tikzset{
%node distance=1.3cm, auto,
%every node/.style={font=\tiny },
%ocenter/.style={baseline={([yshift=-.5ex, xshift=-.5ex]current bounding box)}},  
%labelBeginAbove/.style={postaction={decorate,decoration={markings,mark=at position 0 with {\node[inner sep= 0.6pt, above=1pt]{\tiny #1};}} } },
%labelBeginBelow/.style={postaction={decorate,decoration={markings,mark=at position 0 with {\node[inner sep= 0.6pt, below=1pt]{\tiny #1};}}}},
%labelEndAbove/.style={postaction={decorate,decoration={markings,mark=at position 1 with {\node[inner sep= 0.6pt, above=1pt]{\tiny #1};}}}},
%labelEndBelow/.style={postaction={decorate,decoration={markings,mark=at position 1 with {\node[inner sep= 0.6pt, below=1pt]{\tiny #1};}}}},
%labelEndRight/.style={postaction={decorate,decoration={markings,mark=at position 1 with {\node[inner sep= 0.6pt, right=1pt]{\tiny #1};}}}},
%labelEndLeft/.style={postaction={decorate,decoration={markings,mark=at position 1 with {\node[inner sep= 0.6pt, left=1pt]{\tiny #1};}}}}
%}

\newcommand{\nodeHorDist}{2cm}
\newcommand{\nodeVerDist}{1cm}

\newcommand{\commDiagramRed}[8]{
% Square commuting diagram with arrows
%
% #1-4 nodes in the order North-West NE SW SE
% #5-8 arrows in the order NW-NE SW-SE NW-NE SW-SE

\begin{tikzpicture}[ocenter]
	\node (s) {\normalsize #1};
  \node at (s.center)  [right=1.7*\nodeHorDist](s1){\normalsize #2};
  \node at (s.center)  [below=\nodeVerDist](s2) {\normalsize #3};
  \node at (s1|-s2) (t) {\normalsize #4};
  
  \draw[->] (s) to node {#5} (s1);
  \draw[->] (s2) to node {#6} (t);
  \draw[->] (s) to node {#7} (s2);
  \draw[->] (s1) to node {#8} (t);
\end{tikzpicture} 
}

==> latex-macros/ben-macros-nets.tex <==
%% tikz
\usepackage{tikz}
\usetikzlibrary{calc}
\usetikzlibrary{backgrounds}
\usetikzlibrary{decorations.shapes}
\usetikzlibrary{decorations.text}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{matrix}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{arrows}
\usetikzlibrary{positioning}
\usepackage[nofancy]{tikz-inet}

\setboolean{withimages}{true}

\tikzset{%
%
% tikzpictures
  ocenter/.style={baseline={([yshift=-.5ex, xshift=-.5ex]current bounding box)}},  
%
% NODE STYLES
  nospace/.style={inner sep= 0pt},
  etic/.style={inner sep= 0.5pt, fill=white, anchor= center},
  letic/.style={inner sep= 0.7pt, fill=white, anchor= center,circle,draw=black},
%
% MELL nets  
  port/.style={inner sep= 0.3pt, anchor= center,circle,draw=black,fill=black, minimum size = 0.3pt},
%
% cbv nets  
  eport/.style={inner sep= 0.8pt, anchor= center,circle,draw=cyan,fill=white, minimum size = 0.8pt},
  mport/.style={inner sep= 0.8pt, anchor= center, circle,draw=white,fill=brown, minimum size = 0.8pt, solid, 
line width=0.10ex},
% cbn nets  
  eportn/.style={inner sep= 0.8pt, anchor= center,circle,draw=blue,fill=white, minimum size = 0.8pt},
  mportn/.style={inner sep= 0.8pt, anchor= center, circle,draw=red,fill=red, minimum size = 0.8pt, solid, 
line width=0.10ex},
%
%
% EDGE STYLES
  nopol/.style={->, shorten <=0.5pt, shorten >=0.5pt, draw=gray, line width=0.18ex},
  nopolrev/.style={<-, shorten <=1pt, shorten >=1pt, draw=gray, line width=0.18ex},
  nopolgen/.style={preaction={decorate},decoration={markings,mark=at position .5 with {\draw [shorten >=0pt, shorten <=0pt,draw=gray,-](0pt,3pt) -- (0pt,-3pt);}},->, shorten <=0.5pt, shorten >=0.5pt, draw=gray, line width=0.18ex},
  nopolrevgen/.style={preaction={decorate},decoration={markings,mark=at position .5 with {\draw [shorten >=0pt, shorten <=0pt,draw=gray,-](0pt,3pt) -- (0pt,-3pt);}},<-, shorten <=1pt, shorten >=1pt, draw=gray, line width=0.18ex},
  outEdge/.style={<-, shorten >=0.5pt, shorten <=0.5pt, draw=blue, line width=0.18ex},
  inpEdge/.style={->, densely dotted, shorten >=0.5pt, shorten <=0.5pt, draw=red, line width=0.18ex, overlay},
  inpEdgeGen/.style={preaction={decorate},decoration={markings,mark=at position .5 with {\draw [shorten >=0pt, shorten <=0pt,draw=red,-](0pt,3pt) -- (0pt,-3pt);}},->, densely dotted, shorten >=0.5pt, shorten <=0.5pt, draw=red, line width=0.18ex, overlay},
  %
  % cbv nets
    eprinc/.style={postaction={decorate},decoration={markings,mark=at position .4 with {\node [inner sep= 0.5pt, anchor= center,circle,draw=cyan, fill=cyan, minimum size = 0.8pt, solid, line width=0.10ex]{};}}},
    mprinc/.style={postaction={decorate},decoration={markings,mark=at position .4 with {\node [inner sep= 0.5pt, anchor= center,circle,draw=brown, fill=brown, minimum size = 0.8pt, solid, line width=0.10ex]{};}}},
    mprincpar/.style={postaction={decorate},decoration={markings,mark=at position .6 with {\node [inner sep= 0.5pt, anchor= center,circle,draw=brown, fill=brown, minimum size = 0.8pt, solid, line width=0.10ex]{};}}},
    pure/.style={->, shorten <=1pt, shorten >=1pt, draw=brown, line width=0.18ex},
    pureRev/.style={<-, shorten <=1pt, shorten >=1pt, draw=brown, line width=0.18ex},
    exppure/.style={->, shorten <=1pt, shorten >=1pt, draw=cyan, line width=0.18ex, densely dotted},
    exppureRev/.style={<-, shorten <=1pt, shorten >=1pt, draw=cyan, line width=0.18ex, densely dotted},    genexppure/.style={preaction={decorate},decoration={markings,mark=at position .5 with {\draw [shorten >=0pt, shorten <=0pt,draw=cyan,-](0pt,3pt) -- (0pt,-3pt);}},->, shorten <=1pt, shorten >=1pt, draw=cyan, line width=0.18ex, densely dotted},
    enaryedge/.style={preaction={decorate},decoration={markings,mark=at position .5 with {\draw [shorten >=0pt, shorten <=0pt,draw=cyan,-](0pt,3pt) -- (0pt,-3pt);}}},
  % cbn nets
    eprincn/.style={postaction={decorate},decoration={markings,mark=at position .4 with {\node [inner sep= 0.7pt, anchor= center,circle,draw=blue, fill=blue, minimum size = 0.8pt, solid, line width=0.10ex]{};}}},
    mprincn/.style={postaction={decorate},decoration={markings,mark=at position .6 with {\node [inner sep= 0.7pt, anchor= center,circle,draw=red, fill=white, minimum size = 0.8pt, solid, line width=0.10ex]{};}}},
    mprincnpar/.style={postaction={decorate},decoration={markings,mark=at position .4 with {\node [inner sep= 0.7pt, anchor= center,circle,draw=red, fill=white, minimum size = 0.8pt, solid, line width=0.10ex]{};}}},
    puren/.style={->, shorten <=1pt, shorten >=1pt, draw=red, line width=0.18ex},
    purenRev/.style={<-, shorten <=1pt, shorten >=1pt, draw=red, line width=0.18ex},
    exppuren/.style={->, shorten <=1pt, shorten >=1pt, draw=blue, line width=0.18ex, densely dotted},
    exppurenRev/.style={<-, shorten <=1pt, shorten >=1pt, draw=blue, line width=0.18ex, densely dotted},    genexppuren/.style={preaction={decorate},decoration={markings,mark=at position .5 with {\draw [shorten >=0pt, shorten <=0pt,draw=blue,-](0pt,3pt) -- (0pt,-3pt);}},->, shorten <=1pt, shorten >=1pt, draw=blue, line width=0.18ex, densely dotted},
    enaryedge/.style={preaction={decorate},decoration={markings,mark=at position .5 with {\draw [shorten >=0pt, shorten <=0pt,draw=blue,-](0pt,3pt) -- (0pt,-3pt);}}},
%
% BOX LINE STYLES
  jboxline/.style={draw= gray,rounded corners, line width=0.20ex, overlay},
  exboxline/.style={draw= gray,line width=0.20ex, overlay},
  noboxline/.style={draw= white,rounded corners, line width=0ex},
%
% NETS
  net/.style={draw=gray,inner sep=2pt,thick,ellipse, anchor=center, font=\scriptsize},
  inductiveTr/.style={draw=black!50, minimum size=0.9cm},
  inductiveTrSmall/.style={draw=black!50, minimum size=0.6cm},
%
% EVERY
  every label/.style={label distance = 1pt, font=\scriptsize, inner sep= 1pt},  
  every node/.style={font=\scriptsize }%\small
}
%\node[etic,fill=white]{{\tiny 0}}

\newcommand{\altax}{8pt}
\newcommand{\altcut}{8pt}


\newcommand{\staltb}{30pt}
\newcommand{\stlarb}{25pt}
\newcommand{\hstaltb}{\staltb/2}
\newcommand{\hstlarb}{\stlarb/2}

\newcommand{\stalt}{22pt}
\newcommand{\stlar}{15pt}
\newcommand{\hstalt}{\stalt/2}
\newcommand{\hstlar}{\stlar/2}
\newcommand{\hhstalt}{\stalt/4}
\newcommand{\hhstlar}{\stlar/4}

\newcommand{\staltm}{17.8pt}
\newcommand{\stlarm}{13.6pt}
\newcommand{\hstaltm}{\staltm/2}
\newcommand{\hstlarm}{\stlarm/2}

\newcommand{\ilar}{12pt}
\newcommand{\hilar}{\ilar/2}

\newcommand{\auxdistance}{5pt}
\newcommand{\pendingdist}{10pt}
\newcommand{\anchorh}{9pt}
\newcommand{\anchorw}{9pt}

%LINKS
\input{\macrospath/graphical-macros/generic-links}
\input{\macrospath/graphical-macros/links-MELL}

%SEPARATORI
\newcommand{\invsep}[2]{%parametri: #1=larghezza della separazione,
                                                   %#2= altezza del separatore
  \begin{tikzpicture}[ocenter]%separatore
    \node (up){};
    \node at (up.center) [below right=#2 and #1](down){};
  \end{tikzpicture}
}

\newcommand{\sepColonne}[2]{%parametri: #1=larghezza della separazione,
                                                   %#2= altezza del separatore
  \begin{tikzpicture}[ocenter]%separatore
    \node (up){};
    \node at (up) [below=#2](down){};
    \draw [color=gray] (up) to (down);
    \node at (up) [left = #1] (left){};
    \node at (up) [right= #1] (right){};
  \end{tikzpicture}
}

\newcommand{\sepRows}[2]{%parametri: #1=Larghezza della separazione,
                                                   %#2= altezza del separatore
  \begin{tikzpicture}[ocenter]%separatore
    \node (up){};
    \node at (up) [right=#1](down){};
    \draw [color=gray] (up) to (down);
    \node at (up) [above = #2] (left){};
    \node at (up) [below= #2] (right){};
  \end{tikzpicture}
}

\newcommand{\lineasep}{\multicolumn{6}{c}{\sepRows{200pt}{0.5pt}}}
\newcommand{\lineaseplong}{\multicolumn{9}{c}{\sepRows{350pt}{0.5pt}}}

\newcommand{\gdots}[3]{
% 1 = left node
% 2 = right node
% 3 = eventual parameters
\node at ($(#1)!.5!(#2)$) [#3]{\tiny $\ldots$};
}

\newcommand{\gdotsname}[4]{
% 1 = left node
% 2 = right node
% 3 = eventual parameters
% 4 = name of the node
\node at ($(#1)!.5!(#2)$) [#3](#4){\tiny $\ldots$};
}

\newcommand{\bracketup}[5]{
% 1 = left node
% 2 = right node
% 3 = height
% 4 = label
% 5 = name
\node at \med{#1}{#2}[above=#3, nospace](#4){};

\draw[out=90, in=-90] (#1) to (#4);
\draw[out=90, in=-90] (#2) to (#4);
\node at (#4.center)[ above=\sepbox, nospace](#4label){#5};
}

\newcommand{\bracketdown}[5]{
% 1 = left node
% 2 = right node
% 3 = height
% 4 = label
% 5 = name
\node at \med{#1}{#2}[below=#3, nospace](#4){};

\draw[out=-90, in=90] (#1) to (#4);
\draw[out=-90, in=90] (#2) to (#4);
\node at (#4.center)[ below=\sepbox, nospace](#4label){#5};}

\newcommand{\mednop}[2]{
$(#1)!.5!(#2)$
}
